SEEK: Secure and Efficient Encrypted Keyword Search For Privacy-Preserving Messaging Protocols

Encrypted communication protects sensitive user data but can facilitate harmful or unlawful exchanges, creating a trade-off between detecting dangerous messages and preserving end-user privacy. To address this, we propose SEEK, a practical and efficient encrypted keyword-search protocol for privacy-preserving messaging that combines homomorphic encryption with secure two-party computation (2PC). SEEK first partitions messages into ciphertext fragments with the minimum sufficient overlap, then homomorphically correlates them using encrypted keyword trapdoors. For long messages, this design can reduce sender-side encryption and upload overhead by up to two orders of magnitude over state-of-the-art baselines. It supports ASCII case-insensitive matching with one fixed-size encrypted trapdoor and one homomorphic multiplication per fragment, yielding up to 5.47x faster correlation computation than the strongest fragmentation-based baselines. SEEK then invokes 2PC-based selected decoding, blinded zero testing, and secure aggregation, revealing only the keyword presence-or-absence bit while hiding the keyword, its length, message contents, match counts, and locations. SEEK achieves 100% accuracy under case variations that result in exact-matching failures, without requiring additional trapdoors or online communication. We further realize SEEK as an end-to-end web and cross-platform mobile application. Prototype evaluation on a weekly messaging history yields an online computation time of 1.92 s per search, demonstrating the practical feasibility and efficiency of SEEK.

==> Sections/10-Ethics.tex <==
\section*{Ethical Considerations}
\label{sec:ethical-considerations}

End-to-end encryption is essential for keeping private communications safe from cloud providers, outside/insider attackers, and unauthorized access. Still, requests for access during investigations or compliance efforts can create pressure to weaken encryption, compromise endpoints, or grant broad access to plaintext. \ProtocolName{} takes a more focused approach by letting an authorized keyword query run over stored ciphertexts, without giving either party access to plaintext. In the described threat model, $\mathsf{CSP}$ only handles ciphertexts and does not learn the keyword, its length, or the search result. $\mathsf{PP}$ gets a single presence bit for the whole corpus but does not learn any plaintext, correlation value, match count, or match location. The receiver is not involved in the search, and decoding and result aggregation are split between $\mathsf{PP}$ and $\mathsf{CSP}$. These features make \ProtocolName{} a disclosure-minimizing option compared to server-side decryption or endpoint compromise. The protocol does not decide if a search is legal, necessary, proportionate, or ethically justified. Like other search tools, \ProtocolName{} can be used for good or bad purposes, and this work should not be seen as supporting widespread monitoring of encrypted messages. It is meant to add to, not replace, voluntary abuse-reporting and message-franking systems, which are better in presence of an honest recipient.

\noindent \ding{110}
\paragraphNew{\DeepUL{Query Budgets and Collusion}}
\ProtocolName{} assumes that queries are approved and does not link a trapdoor to a warrant, authorized keyword, or policy rule, nor does it enforce a query budget. This means an authorized $\mathsf{PP}$ could make broad, adaptive, or specific queries and use the presence bits to learn information. A budget set by $\mathsf{CSP}$ can limit this only if the two parties do not work together. Our repeated-query analysis looks at the computing and communication costs of such query campaigns, but these costs prohibit exhaustive query attacks. If $\mathsf{PP}$ and $\mathsf{CSP}$ work together, they can get around admission controls, rate limits, and aggregation, even without rebuilding the receiver's secret key or directly decrypting stored ciphertexts. By sharing their decoding and zero-test states, they can remove the protections on individual results, turning the presence interface into a search tool for each position. For example, if one-byte queries are allowed, the two parties can try every ASCII letter at every byte position at once. The matching letter at each spot reveals the plaintext byte, except for case-folding ambiguity, and $\mathsf{CSP}$ can use the corpus layout to map these back to messages and fragments. So, a limited number of well-chosen searches could recover the case-normalized text instead of just one presence bit. Even if some values are not available, unrestricted adaptive dictionary, identifier, phrase, and substring queries can still reveal a lot about predictable data sets. Because of this, query budgets should be enforced by an independent authorization system outside both parties, along with signed approvals, rate limits, and tamper-evident audits. The privacy guarantee does not fundamentally apply if $\mathsf{PP}$ and $\mathsf{CSP}$ collude.

\noindent \ding{110}
\paragraphNew{\DeepUL{Detection and Evidentiary Limits}}
\ProtocolName{} can only find exact ASCII case-insensitive keyword matches if clients use the required encoding and encryption steps. Code words, intentional obfuscation, modified clients, images, and messages encrypted outside the system can avoid detection. Also, finding a keyword does not prove harmful intent, context, or legal responsibility. A positive result should be seen as an investigative lead that needs independent review, not as sufficient evidence for an automated negative decision.

\noindent \ding{110}
\paragraphNew{\DeepUL{Deployment Safeguards}}
Responsible deployment needs protections that go beyond what the cryptographic protocol provides. These include independent authorization and approval from multiple parties for each search, ways to link allowed trapdoors to approved rules, strong authentication, signed and tamper-evident query records, limits per user and investigation, rate limiting, anomaly detection, independent audits, transparency reports, and proper legal review and redress. Deployments should also keep $\mathsf{PP}$ and $\mathsf{CSP}$ separate, protect key storage, rotate keys, support revocation and incident response, use short retention periods, and securely erase expired ciphertexts and secret-key shares. These are deployment requirements, not guarantees that \ProtocolName{} currently provides. Cryptographic efficiency cannot replace legal, organizational, and human rights review.

\noindent \ding{110}
\paragraphNew{\DeepUL{Research Data and Disclosure}}
Our evaluation did not include any human participants, user studies, deception, or collection of private user messages. We used publicly available benchmark data, such as \textsf{SAMSum} and the listed word-frequency resources, along with synthetic and adversarial test inputs. As a result, the study did not involve human subjects research that would require institutional review. We also did not find or test any vulnerability in a deployed system, so coordinated vulnerability disclosure was not needed.

==> Sections/11-OpenScience.tex <==


\section*{Open Science}

We provide an anonymized artifact with complete running instructions at \url{https://anonymous.4open.science/r/SEEK-USENIX}. Its evaluation component reproduces the results in Sections~\ref{sec:eval_microbenchmarks} and~\ref{sec:eval_repeated_queries}, including the 20-profile, 10-workload campaign, correctness, preprocessing, communication, repeated-query, and baseline~\cite{1} experiments, as well as the BFV validation in Appendix~\ref{app:bfv-params}. The optimized proof-of-concept web/mobile application produces the prototype measurements in Section~\ref{sec:eval_prototype} and is illustrated in Appendix~\ref{applicationImages}. A separate Dockerized application demonstrates the complete workflow while recording full-stack timings that include application and orchestration overhead rather than the strict \ProtocolName{}-only measurements used in the paper. Each component includes a README detailing its dependencies, setup, execution, testing, and result collection. Third-party datasets and word-frequency resources are not redistributed, and the evaluation README explains how to obtain and install them. Wall-clock measurements may vary with the hardware.


